ATHENA: A Framework based on Diverse Weak Defenses for Building Adversarial Defense

There has been extensive research on developing defense techniques against adversarial attacks; however, they have been mainly designed for specific model families or application domains, therefore, they cannot be easily extended. Based on the design philosophy of ensemble of diverse weak defenses, we propose ATHENA---a flexible and extensible framework for building generic yet effective defenses against adversarial attacks. We have conducted a comprehensive empirical study to evaluate several realizations of ATHENA with four threat models including zero-knowledge, black-box, gray-box, and white-box. We also explain (i) why diversity matters, (ii) the generality of the defense framework, and (iii) the overhead costs incurred by ATHENA.

==> tables/architects.tex <==
\begin{tabular}{ll}
\toprule
Table & to fill \\
\midrule
Architectures of & Models \\
\bottomrule
\end{tabular}


==> tables/attack_config.tex <==
\begin{tabular}{l|c|ll}
\toprule
Attack              &                   &   MNIST                               &   CIFAR-100   \\
\midrule
\FGSM               & $\epsilon$        & $0.1, 0.15, 0.2, 0.25, 0.3$           & $0.002, 0.003, 0.005, 0.0075, 0.03$   \\
\midrule
\BIM~($l_2$)        & $\epsilon$        & $0.75, 0.85, 1, 1.1, 1.2$             & $0.05, 0.75, 0.125, 0.3, 0.5$         \\
\midrule
\BIM~($l_{\infty}$) & $\epsilon$        & $0.0075, 0.0082, 0.009, 0.1, 0.12$    & $0.0025, 0.005, 0.0075, 0.01, 0.015$   \\
\midrule
\CW~($l_2$)         & $lr$              & $0.0098, 0.01, 0.012, 0.015, 0.018$   & $0.0003, 0.001, 0.007, 0.02, 1$        \\
\midrule
\JSMA               & $\theta$          & $0.15,~0.17,~0.018,~0.21,~0.25$       & $0.01,~0.5,~~0.25,~-0.5,~-0.3$  \\ 
                    & $\gamma$          & $0.5,~~0.5,~~~0.5,~~~0.5,~~~0.5$      & $0.04,~0.03,~0.05,~0.075,~~0.1$   \\
\midrule
\PGD                & $\epsilon$        & $0.075, 0.082, 0.09, 0.1, 0.11$       & $0.0015, 0.0025, 0.0035, 0.005, 0.015$ \\
\midrule
\DF                 & $os$              & $3, 5, 8, 16, 50$                     &   \\
\midrule
\OP                 & $pc$              & $15, 30, 35, 40, 75$                  &   \\
\midrule
\MIM                & $\epsilon$        & $0.06, 0.067, 0.075, 0.085, 0.1$      &   \\
\bottomrule
\end{tabular}



==> tables/defense_acc.tex <==
\begin{tabular}{lllll}
\toprule
Defense   & Attack1 & Attack2 & Attack3 & Attack4 \\
\midrule
Random    & xx      & xx      & xxx     & xx      \\ 
CV\_Maj & xxx     & xx      & xxx     & xx      \\ 
CV\_Max & xxx     & x       & xxx     & x       \\ 
1s\_Mean & xx      & x       & xx      & xx      \\
1s\_Mean\_L & xx      & xx      & xx      & x       \\
AdvTrain1 & xxx     & xx      & x       & xx      \\
AdvTrain2 & xxx     & x       & xx      & xx      \\
\bottomrule
\end{tabular}

==> tables/defense_acc_mean.tex <==
\iffalse
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
SampleType                          & $M_{target}$  & CV\_Maj & CV\_Max & 1s\_Mean & EM\_Mean & EM\_MXMV & 1s\_Mean\_L & EM\_Mean\_L & EM\_MXMV\_L \\ \hline
BS                                  & 0.9901        & 0.9915  & 0.9917  & 0.99     & 0.9743   & 0.9716   & 0.9897      & 0.9603      & 0.971       \\ \hline
JSMA ($\theta:0.3, \gamma:0.5$)     & 0.0206        & 0.9849  & 0.9824  & 0.9813   & 0.9456   & 0.9439   & 0.9819      & 0.9337      & 0.9427      \\ \hline
JSMA ($\theta:0.5, \gamma:0.7$)     & 0.0012        & 0.9548  & 0.9375  & 0.9347   & 0.8917   & 0.8878   & 0.938       & 0.8839      & 0.8797      \\ \hline
FGSM ($\epsilon:0.1$)               & 0.7469        & 0.984   & 0.9855  & 0.9834   & 0.9593   & 0.9583   & 0.9828      & 0.9463      & 0.9568      \\ \hline
FGSM ($\epsilon:0.25$)              & 0.171         & 0.8238  & 0.8698  & 0.8729   & 0.8262   & 0.8251   & 0.8752      & 0.8245      & 0.8353      \\ \hline
FGSM ($\epsilon:0.3$)               & 0.1115        & 0.6036  & 0.7154  & 0.7226   & 0.6718   & 0.6677   & 0.7292      & 0.6793      & 0.6786      \\ \hline
BIM ($l^2, \epsilon:0.5$)           & 0.9505        & 0.9909  & 0.9907  & 0.9895   & 0.9774   & 0.9762   & 0.9856      & 0.9543      & 0.968       \\ \hline
BIM ($l^2, \epsilon:1.$)            & 0.7499        & 0.9865  & 0.9874  & 0.986    & 0.9703   & 0.9693   & 0.9856      & 0.951       & 0.9608      \\ \hline
BIM ($l^{\infty}, \epsilon:0.25$)   & 0.0079        & 0.8692  & 0.8967  & 0.9146   & 0.8749   & 0.8703   & 0.9141      & 0.869       & 0.8756      \\ \hline
BIM ($l^{\infty}, \epsilon:0.5$)    & 0.0079        & 0.2568  & 0.3417  & 0.3577   & 0.3245   & 0.3267   & 0.3588      & 0.3304      & 0.3384      \\ \hline
PGD ($\epsilon:0.25$)               & 0.2387        & 0.7896  & 0.8462  & 0.8787   & 0.8356   & 0.8361   & 0.8791      & 0.8233      & 0.8386      \\ \hline
PGD ($\epsilon:0.5$)                & 0.0157        & 0.1493  & 0.2854  & 0.3221   & 0.2916   & 0.3072   & 0.3373      & 0.2975      & 0.3142      \\ \hline
PGD ($\epsilon:0.75$)               & 0.0117        & 0.0513  & 0.0956  & 0.098    & 0.0998   & 0.1132   & 0.1018      & 0.1         & 0.1242      \\ \hline
DF ($maxIter:100$)                  & 0.8407        & 0.9293  & 0.9358  & 0.9397   & 0.9029   & 0.9051   & 0.938       & 0.8842      & 0.8993      \\ \hline
DF ($maxIter:10000$)                & 0.8407        & 0.9296  & 0.9358  & 0.9397   & 0.9028   & 0.9057   & 0.9379      & 0.8842      & 0.8993      \\ \hline
\end{tabular}
\fi

\begin{tabular}{llllll}
\toprule
SampleType                          & $f_{t_0}$     & CV\_Maj & CV\_Max & 1s\_Mean & 1s\_Mean\_L \\
\midrule
BS                                  & 0.9901        & 0.9915  & 0.9917  & 0.99     & 0.9897      \\
JSMA ($\theta:0.3, \gamma:0.5$)     & 0.0206        & 0.9849  & 0.9824  & 0.9813   & 0.9819      \\
JSMA ($\theta:0.5, \gamma:0.7$)     & 0.0012        & 0.9548  & 0.9375  & 0.9347   & 0.938       \\
FGSM ($\epsilon:0.1$)               & 0.7469        & 0.984   & 0.9855  & 0.9834   & 0.9828      \\
FGSM ($\epsilon:0.25$)              & 0.171         & 0.8238  & 0.8698  & 0.8729   & 0.8752      \\
FGSM ($\epsilon:0.3$)               & 0.1115        & 0.6036  & 0.7154  & 0.7226   & 0.7292      \\
BIM ($l^2, \epsilon:0.5$)           & 0.9505        & 0.9909  & 0.9907  & 0.9895   & 0.9856      \\
BIM ($l^2, \epsilon:1.$)            & 0.7499        & 0.9865  & 0.9874  & 0.986    & 0.9856      \\
BIM ($l^{\infty}, \epsilon:0.25$)   & 0.0079        & 0.8692  & 0.8967  & 0.9146   & 0.9141      \\
BIM ($l^{\infty}, \epsilon:0.5$)    & 0.0079        & 0.2568  & 0.3417  & 0.3577   & 0.3588      \\
PGD ($\epsilon:0.25$)               & 0.2387        & 0.7896  & 0.8462  & 0.8787   & 0.8791      \\
PGD ($\epsilon:0.5$)                & 0.0157        & 0.1493  & 0.2854  & 0.3221   & 0.3373      \\
PGD ($\epsilon:0.75$)               & 0.0117        & 0.0513  & 0.0956  & 0.098    & 0.1018      \\
DF ($maxIter:100$)                  & 0.8407        & 0.9293  & 0.9358  & 0.9397   & 0.938       \\
DF ($maxIter:10000$)                & 0.8407        & 0.9296  & 0.9358  & 0.9397   & 0.9379      \\
\bottomrule
\end{tabular}


==> tables/defense_acc_std.tex <==
\iffalse
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
SampleType                        & CV\_Maj & CV\_Max & 1s\_Mean & EM\_Mean & EM\_MXMV & 1s\_Mean\_L & EM\_Mean\_L & EM\_MXMV\_L \\ \hline
BS                                & 0.0054  & 0.0021  & 0.0067   & 0.0414   & 0.0589   & 0.007       & 0.062       & 0.048       \\ \hline
JSMA ($\theta:0.3, \gamma:0.5$)            & 0.0086  & 0.0112  & 0.0161   & 0.0873   & 0.0961   & 0.0128      & 0.1103      & 0.1016      \\ \hline
JSMA ($\theta:0.5, \gamma:0.7$)            & 0.01    & 0.0269  & 0.0308   & 0.1094   & 0.1153   & 0.0245      & 0.1283      & 0.1226      \\ \hline
FGSM ($\epsilon:0.1$)                      & 0.0079  & 0.0032  & 0.0093   & 0.0547   & 0.0655   & 0.0104      & 0.078       & 0.0663      \\ \hline
FGSM ($\epsilon:0.25$)                      & 0.0426  & 0.0838  & 0.0732   & 0.1128   & 0.1132   & 0.0705      & 0.1139      & 0.1027      \\ \hline
FGSM ($\epsilon:0.3$)                      & 0.1238  & 0.177   & 0.1826   & 0.1756   & 0.1698   & 0.1732      & 0.17        & 0.1662      \\ \hline
BIM ($l^2, \epsilon:0.5$)      & 0.0052  & 0.0026  & 0.006    & 0.0291   & 0.0368   & 0.0131      & 0.0646      & 0.0534      \\ \hline
BIM ($l^2, \epsilon:1.$)     & 0.0052  & 0.0026  & 0.0066   & 0.0369   & 0.0434   & 0.0067      & 0.0727      & 0.0631      \\ \hline
BIM ($l^{\infty}, \epsilon:0.25$)    & 0.0284  & 0.0621  & 0.0383   & 0.0839   & 0.0909   & 0.0383      & 0.0922      & 0.086       \\ \hline
BIM ($l^{\infty}, \epsilon:0.5$)    & 0.1245  & 0.1966  & 0.2038   & 0.1817   & 0.1902   & 0.212       & 0.1768      & 0.1961      \\ \hline
PGD ($\epsilon:0.25$) & 0.0388  & 0.0847  & 0.0571   & 0.0916   & 0.093    & 0.0588      & 0.1017      & 0.0957      \\ \hline
PGD ($\epsilon:0.5$) & 0.0956  & 0.2278  & 0.22     & 0.1962   & 0.2097   & 0.2337      & 0.195       & 0.2156      \\ \hline
PGD ($\epsilon:0.75$) & 0.0126  & 0.0614  & 0.0552   & 0.0551   & 0.0572   & 0.0547      & 0.0549      & 0.064       \\ \hline
DF ($maxIter:100$)              & 0.0108  & 0.0134  & 0.0249   & 0.0867   & 0.0889   & 0.0272      & 0.1125      & 0.102       \\ \hline
DF ($maxIter:10000$)            & 0.0109  & 0.0133  & 0.025    & 0.0867   & 0.0891   & 0.0272      & 0.1126      & 0.1019      \\ \hline
\end{tabular}
\fi

\begin{tabular}{lllllllll}
\toprule
SampleType                        	& CV\_Maj & CV\_Max & 1s\_Mean & 1s\_Mean\_L \\
\midrule
BS                                	& 0.0054  & 0.0021  & 0.0067   & 0.007       \\
JSMA ($\theta:0.3, \gamma:0.5$)     & 0.0086  & 0.0112  & 0.0161   & 0.0128      \\
JSMA ($\theta:0.5, \gamma:0.7$)     & 0.01    & 0.0269  & 0.0308   & 0.0245      \\
FGSM ($\epsilon:0.1$)               & 0.0079  & 0.0032  & 0.0093   & 0.0104      \\
FGSM ($\epsilon:0.25$)              & 0.0426  & 0.0838  & 0.0732   & 0.0705      \\
FGSM ($\epsilon:0.3$)               & 0.1238  & 0.177   & 0.1826   & 0.1732      \\
BIM ($l^2, \epsilon:0.5$)      		& 0.0052  & 0.0026  & 0.006    & 0.0131      \\
BIM ($l^2, \epsilon:1.$)     		& 0.0052  & 0.0026  & 0.0066   & 0.0067      \\
BIM ($l^{\infty}, \epsilon:0.25$)   & 0.0284  & 0.0621  & 0.0383   & 0.0383      \\
BIM ($l^{\infty}, \epsilon:0.5$)    & 0.1245  & 0.1966  & 0.2038   & 0.212       \\
PGD ($\epsilon:0.25$) 				& 0.0388  & 0.0847  & 0.0571   & 0.0588      \\
PGD ($\epsilon:0.5$) 				& 0.0956  & 0.2278  & 0.22     & 0.2337      \\
PGD ($\epsilon:0.75$) 				& 0.0126  & 0.0614  & 0.0552   & 0.0547      \\
DF ($maxIter:100$)              	& 0.0108  & 0.0134  & 0.0249   & 0.0272      \\
DF ($maxIter:10000$)            	& 0.0109  & 0.0133  & 0.025    & 0.0272      \\
\bottomrule
\end{tabular}

==> tables/eval_mnist_zk.tex <==
\begin{tabular}{l||l|ll|lllll||lll}
\toprule
\textbf{Model}            & \textbf{UM} & \textbf{PGD-ADT} & \textbf{RS} & \textbf{RD} & \textbf{MV}     & \textbf{AVEP}   & \textbf{T2MV} & \textbf{AVEL}   & \textbf{Gap(UM)} & \textbf{Gap(PGD-ADT)} & \textbf{Gap(RS)} \\ 
\midrule
BS               & 0.9901      & 0.9911            & 0.9824      & 0.9869      & 0.9939          & \textbf{0.9943} & 0.9914        & \textbf{0.9943} & 0.42\%           & 0.32\%                 & 1.21\%           \\
\midrule
FGSM($\epsilon$:0.1)   & 0.7469      & 0.9811            & 0.9662      & 0.9509      & 0.9886          & 0.9895          & 0.9868        & \textbf{0.9903} & 32.59\%          & 0.94\%                 & 2.49\%           \\
FGSM($\epsilon$:0.15)   & 0.4827      & 0.9678            & 0.9427      & 0.9024      & 0.9775          & 0.9819          & 0.975         & \textbf{0.983}  & 103.65\%         & 1.57\%                 & 4.27\%           \\
FGSM($\epsilon$:0.2)    & 0.2845      & 0.9388            & 0.8933      & 0.8054      & 0.9462          & \textbf{0.962}  & 0.9408        & 0.9619          & 238.14\%         & 2.47\%                 & 7.69\%           \\
FGSM($\epsilon$:0.25)   & 0.171       & 0.8656            & 0.799       & 0.6377      & 0.8375          & 0.8983          & 0.8384        & \textbf{0.9041} & 428.71\%         & 4.45\%                 & 13.15\%          \\
FGSM($\epsilon$:0.3)    & 0.1115      & 0.7218            & 0.6664      & 0.4671      & 0.5469          & 0.7242          & 0.5687        & \textbf{0.7701} & 590.67\%         & 6.69\%                 & 15.56\%          \\
\midrule
BIM\_$l_2$($\epsilon$:0.75)  & 0.6179      & 0.9822            & 0.9722      & 0.9608      & \textbf{0.9894} & 0.9648          & 0.9876        & 0.9657          & 60.12\%          & 0.73\%                 & 1.77\%           \\
BIM\_$l_2$($\epsilon$:0.85)  & 0.4702      & 0.9802            & 0.9688      & 0.9487      & \textbf{0.9869} & 0.9733          & 0.9846        & 0.9752          & 109.89\%         & 0.68\%                 & 1.87\%           \\
BIM\_$l_2$($\epsilon$:1)     & 0.2574      & 0.9765            & 0.9631      & 0.9395      & \textbf{0.9828} & 0.9801          & 0.978         & 0.9827          & 281.82\%         & 0.65\%                 & 2.05\%           \\
BIM\_$l_2$($\epsilon$:1.1)   & 0.1443      & 0.9728            & 0.9598      & 0.9298      & 0.9801          & 0.9798          & 0.971         & \textbf{0.9825} & 580.87\%         & 1.00\%                 & 2.37\%           \\
BIM\_$l_2$($\epsilon$:1.2)   & 0.0772      & 0.9683            & 0.9548      & 0.9225      & 0.9757          & 0.9788          & 0.9635        & \textbf{0.9831} & 1173.45\%        & 1.53\%                 & 2.96\%           \\
\midrule
BIM\_$l_{\infty}$($\epsilon$:0.075) & 0.6043      & 0.9841            & 0.9715      & 0.9517      & 0.9899          & 0.9908          & 0.9884        & \textbf{0.9916} & 64.09\%          & 0.76\%                 & 2.07\%           \\
BIM\_$l_{\infty}$($\epsilon$:0.082) & 0.4672      & 0.9831            & 0.9693      & 0.9478      & 0.9894          & 0.99            & 0.9868        & \textbf{0.9913} & 112.18\%         & 0.83\%                 & 2.27\%           \\
BIM\_$l_{\infty}$($\epsilon$:0.09)  & 0.3159      & 0.9817            & 0.969       & 0.939       & 0.9881          & 0.9889          & 0.9839        & \textbf{0.9902} & 213.45\%         & 0.87\%                 & 2.19\%           \\
BIM\_$l_{\infty}$($\epsilon$:0.1)   & 0.1727      & 0.979             & 0.9629      & 0.9311      & 0.9857          & 0.9882          & 0.9819        & \textbf{0.9885} & 472.38\%         & 0.97\%                 & 2.66\%           \\
BIM\_$l_{\infty}$($\epsilon$:0.12)  & 0.0343      & 0.9745            & 0.9556      & 0.9021      & 0.9814          & 0.9853          & 0.9719        & \textbf{0.9857} & 2773.76\%        & 1.15\%                 & 3.15\%           \\
\midrule
CW\_$l_2$(lr:0.0098)  & 0.3947      & 0.9876            & 0.9746      & 0.974       & \textbf{0.9941} & 0.9646          & 0.993         & 0.9636          & 151.86\%         & 0.66\%                 & 2.00\%           \\
CW\_$l_2$(lr:0.01)    & 0.3763      & 0.9874            & 0.9753      & 0.9746      & \textbf{0.994}  & 0.9633          & 0.993         & 0.9626          & 164.15\%         & 0.67\%                 & 1.92\%           \\
CW\_$l_2$(lr:0.012)   & 0.2379      & 0.9878            & 0.9726      & 0.9728      & \textbf{0.9939} & 0.9544          & 0.9932        & 0.9535          & 317.78\%         & 0.62\%                 & 2.19\%           \\
CW\_$l_2$(lr:0.015)   & 0.1278      & 0.9877            & 0.9729      & 0.9713      & \textbf{0.9939} & 0.9472          & 0.9929        & 0.9464          & 677.70\%         & 0.63\%                 & 2.16\%           \\
CW\_$l_2$(lr:0.018)   & 0.0806      & 0.9871            & 0.9711      & 0.9692      & \textbf{0.994}  & 0.9371          & 0.9931        & 0.9359          & 1133.25\%        & 0.70\%                 & 2.36\%           \\
\midrule
DF(os:3)         & 0.6731      & 0.9777            & 0.9673      & 0.9473      & \textbf{0.984}  & 0.9292          & 0.9823        & 0.9324          & 46.19\%          & 0.64\%                 & 1.73\%           \\
DF(os:5)         & 0.4522      & 0.9479            & 0.938       & 0.8748      & \textbf{0.9531} & 0.9368          & 0.9489        & 0.9475          & 110.77\%         & 0.55\%                 & 1.61\%           \\
DF(os:8)         & 0.3268      & 0.866             & 0.8668      & 0.719       & 0.7923          & 0.8305          & 0.8029        & \textbf{0.8786} & 168.85\%         & 1.45\%                 & 1.36\%           \\
DF(os:16)        & 0.2243      & \textbf{0.5842}   & 0.581       & 0.4558      & 0.4406          & 0.4835          & 0.4508        & 0.5801          & 158.63\%         & -0.70\%                & -0.15\%          \\
DF(os:50)        & 0.154       & 0.251             & 0.2496      & 0.2359      & 0.254           & \textbf{0.2581} & 0.2483        & 0.255           & 67.60\%          & 2.83\%                 & 3.41\%           \\
\midrule
JSMA($\theta$:0.15) & 0.625       & 0.9899            & 0.9781      & 0.9434      & 0.9936          & \textbf{0.9945} & 0.9931        & 0.9935          & 59.12\%          & 0.46\%                 & 1.68\%           \\
JSMA($\theta$:0.17) & 0.4548      & 0.9894            & 0.977       & 0.9414      & 0.993           & \textbf{0.9934} & 0.992         & 0.9924          & 118.43\%         & 0.40\%                 & 1.68\%           \\
JSMA($\theta$:0.18) & 0.3799      & 0.9878            & 0.9768      & 0.9356      & 0.9931          & \textbf{0.9936} & 0.993         & 0.9931          & 161.54\%         & 0.59\%                 & 1.72\%           \\
JSMA($\theta$:0.21) & 0.1874      & 0.9885            & 0.9753      & 0.9319      & 0.993           & \textbf{0.9931} & 0.9918        & 0.9915          & 429.94\%         & 0.47\%                 & 1.83\%           \\
JSMA($\theta$:0.25) & 0.0706      & 0.9873            & 0.9719      & 0.9216      & 0.9915          & \textbf{0.9924} & 0.9899        & 0.9902          & 1305.67\%        & 0.52\%                 & 2.11\%           \\
\midrule
MIM($\epsilon$:0.06)    & 0.699       & 0.9856            & 0.975       & 0.9609      & 0.9912          & 0.9923          & 0.9898        & \textbf{0.9924} & 41.97\%          & 0.69\%                 & 1.78\%           \\
MIM($\epsilon$:0.067)   & 0.5794      & 0.9843            & 0.9727      & 0.9581      & 0.9907          & 0.9913          & 0.988         & \textbf{0.9919} & 71.19\%          & 0.77\%                 & 1.97\%           \\
MIM($\epsilon$:0.075)   & 0.4266      & 0.9841            & 0.9715      & 0.945       & 0.9898          & 0.9904          & 0.9872        & \textbf{0.9914} & 132.40\%         & 0.74\%                 & 2.05\%           \\
MIM($\epsilon$:0.085)   & 0.2509      & 0.9804            & 0.9672      & 0.9389      & 0.9885          & 0.9891          & 0.9825        & \textbf{0.9908} & 294.90\%         & 1.06\%                 & 2.44\%           \\
MIM($\epsilon$:0.1)     & 0.0636      & 0.9784            & 0.9608      & 0.9191      & 0.9839          & 0.9867          & 0.9782        & \textbf{0.988}  & 1453.46\%        & 0.98\%                 & 2.83\%           \\
\midrule
OP(pc:15)        & 0.69        & 0.9685            & 0.9698      & 0.9215      & 0.9826          & 0.9867          & 0.9796        & \textbf{0.9893} & 43.38\%          & 2.15\%                 & 2.01\%           \\
OP(pc:30)        & 0.5111      & 0.9568            & 0.9622      & 0.8795      & 0.9752          & 0.9843          & 0.9654        & \textbf{0.9876} & 93.23\%          & 3.22\%                 & 2.64\%           \\
OP(pc:35)        & 0.4403      & 0.9486            & 0.9582      & 0.8635      & 0.9741          & 0.9821          & 0.9625        & \textbf{0.9872} & 124.21\%         & 4.07\%                 & 3.03\%           \\
OP(pc:40)        & 0.377       & 0.9446            & 0.9545      & 0.8459      & 0.9705          & 0.9829          & 0.9551        & \textbf{0.9882} & 162.12\%         & 4.62\%                 & 3.53\%           \\
OP(pc:75)        & 0.1665      & 0.9023            & 0.9171      & 0.7414      & 0.929           & 0.9658          & 0.8952        & \textbf{0.9804} & 488.83\%         & 8.66\%                 & 6.90\%           \\
\midrule
PGD($\epsilon$:0.075)   & 0.5889      & 0.9839            & 0.9719      & 0.9509      & 0.9905          & 0.9908          & 0.9882        & \textbf{0.9914} & 68.35\%          & 0.76\%                 & 2.01\%           \\
PGD($\epsilon$:0.082)   & 0.3188      & 0.9824            & 0.9707      & 0.9443      & 0.9895          & 0.99            & 0.9857        & \textbf{0.9912} & 210.92\%         & 0.90\%                 & 2.11\%           \\
PGD($\epsilon$:0.09)    & 0.2848      & 0.9806            & 0.9667      & 0.9371      & 0.9878          & 0.9894          & 0.9844        & \textbf{0.9904} & 247.75\%         & 1.00\%                 & 2.45\%           \\
PGD($\epsilon$:0.1)     & 0.1431      & 0.9793            & 0.9641      & 0.9302      & 0.9855          & 0.9877          & 0.9806        & \textbf{0.9894} & 591.40\%         & 1.03\%                 & 2.62\%           \\
PGD($\epsilon$:0.11)    & 0.045       & 0.9772            & 0.9617      & 0.924       & 0.9846          & 0.9859          & 0.9761        & \textbf{0.9875} & 2094.44\%        & 1.05\%                 & 2.68\%           \\ 
\bottomrule
\end{tabular}


==> tables/mnist_norms_defensesize.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{lllllll}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{l}{$l^0$ norm} & \multicolumn{2}{l}{$l^2$ norm} & \multicolumn{2}{l}{$l^{\infty}$ norm} \\ \cline{2-7} 
                       & norm      & count      & norm      & count      & norm      & count      \\
\midrule
trans1                 & xxx       & n                & xxx       & n                & xx        & n                \\
trans2                 & xxx       & n                & xxx       & n                & xx        & n                \\
trans3                 & xxx       & n                & xxx       & n                & xxx       & n                \\
trans4                 & xxx       & n                & xxx       & n                & xx        & n                \\
trans5                 & xx        & n                & xx        & n                & xxx       & n                \\
trans6                 & xx        & n                & xx        & n                & xx        & n                \\
trans7                 & xxxx      & n                & xxxx      & n                & xxx       & n                \\
trans8                 & xx        & n                & xx        & n                & xxx       & n                \\
trans9                 & xxx       & n                & xxx       & n                & xxx       & n                \\
\bottomrule
\end{tabular}

==> tables/mnist_single_test_acc.tex <==
\begin{tabular}{lllll}
\toprule
Model                         & clean  & \begin{tabular}[c]{@{}l@{}}PGD \\ $\epsilon = 0.25$\end{tabular} & \begin{tabular}[c]{@{}l@{}}PGD \\ $\epsilon = 0.50$\end{tabular} & \begin{tabular}[c]{@{}l@{}}PGD \\ $\epsilon = 0.75$\end{tabular} \\
\midrule
BS                              & 0.9901 & 0.2387      & 0.0157      & 0.0117      \\ 
compress\_both                  & 0.9914 & 0.6915      & 0.1208      & 0.0654      \\
stretch\_both                   & 0.9896 & 0.5606      & 0.1003      & 0.0625      \\
compress\_horizontal            & 0.9902 & 0.5633      & 0.1465      & 0.0724      \\
stretch\_horizontal             & 0.9905 & 0.6397      & 0.1024      & 0.0664      \\
compress\_vertical              & 0.99   & 0.697       & 0.1241      & 0.0641      \\
stretch\_vertical               & 0.9885 & 0.6116      & 0.0821      & 0.0543      \\
distortion\_x                   & 0.9884 & 0.6596      & 0.1163      & 0.0499      \\
distortion\_y                   & 0.9879 & 0.8124      & 0.1313      & 0.0514      \\
feature\_std\_norm              & 0.9814 & 0.4708      & 0.0514      & 0.0111      \\
filter\_gaussian                & 0.9907 & 0.4406      & 0.1315      & 0.0696      \\
\bottomrule
\end{tabular}


==> tables/nn_arch_cifar100.tex <==
\footnotesize{
\begin{tabular}{llll}
\toprule
Architecture       &        &   Parameters          &           \\
\midrule
network  & Wide ResNet    &   optimizer &   SGD    \\
depth & $28$         &   learning rate       &   0.1   \\
$k$   & $10$    &   batch size          &   128     \\
    &          &   epoch              &   200      \\
    &           &   lr scheduler    & cosine    \\
\bottomrule
\end{tabular}
}



==> tables/perturbed_norms.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{Model} & \multicolumn{2}{l|}{$l^0$ norm} & \multicolumn{2}{l|}{$l^2$ norm} & \multicolumn{2}{l|}{$l^{\infty}$ norm} \\ \cline{2-7} 
                       & norm      & \#\_of\_def      & norm      & \#\_of\_def      & norm      & \#\_of\_def      \\ \hline
trans1                 & xxx       & n                & xxx       & n                & xx        & n                \\ \hline
trans2                 & xxx       & n                & xxx       & n                & xx        & n                \\ \hline
trans3                 & xxx       & n                & xxx       & n                & xxx       & n                \\ \hline
trans4                 & xxx       & n                & xxx       & n                & xx        & n                \\ \hline
trans5                 & xx        & n                & xx        & n                & xxx       & n                \\ \hline
trans6                 & xx        & n                & xx        & n                & xx        & n                \\ \hline
trans7                 & xxxx      & n                & xxxx      & n                & xxx       & n                \\ \hline
trans8                 & xx        & n                & xx        & n                & xxx       & n                \\ \hline
trans9                 & xxx       & n                & xxx       & n                & xxx       & n                \\ \hline
\end{tabular}

==> tables/rq2/ensembles_acc.tex <==
\begin{tabular}{lccccccccc}
\toprule
   & $f$ & $f_{ens}$ (I/10) & $f_{ens}$ (I/30) & $f_{ens}$ (I/50)  & $f_{ens}$ (I/70) & $f_{ens}$ (II/10) & $f_{ens}$ (II/30) & $f_{ens}$ (II/50)  & $f_{ens}$ (II/70) \\
\midrule
No attack   & xx      & xx      & xxx     & xx      & xx      & xx      & xxx     & xx      & xx \\
Attack 1    & xx      & xx      & xxx     & xx      & xx      & xx      & xxx     & xx      & xx \\ 
Attack 2    & xx      & xx      & xxx     & xx      & xx      & xx      & xxx     & xx      & xx \\ 
Attack 3    & xx      & xx      & xxx     & xx      & xx      & xx      & xxx     & xx      & xx \\ 
Attack 4    & xx      & xx      & xxx     & xx      & xx      & xx      & xxx     & xx      & xx \\ 
Attack 5    & xx      & xx      & xxx     & xx      & xx      & xx      & xxx     & xx      & xx \\ 
Attack 6    & xx      & xx      & xxx     & xx      & xx      & xx      & xxx     & xx      & xx \\ 
Attack 7    & xx      & xx      & xxx     & xx      & xx      & xx      & xxx     & xx      & xx \\ 
\bottomrule
\end{tabular}

==> tables/training_configs.tex <==
\footnotesize{
\begin{tabular}{lll}
\toprule
Parameters          & MNIST & CIFAR                                                                \\
\midrule
Optimization Method & Adam  & RMSprop                                                              \\
Learning Rate       & 0.001 & Scheduled LR                                                         \\
Batch Size          & 128   & 64                                                                   \\
Epochs              & 50    & 100                                                                  \\
Data Augmentation   & ---   & Rotation + Vertical Shifting \\
                            && + Horizontal Shifting + Horizontal Flip \\
\bottomrule
\end{tabular}
}
